Likelihood-based inference for partially observed stochastic epidemics with individual heterogeneity

We develop a stochastic epidemic model progressing over dynamic networks, where infection rates are heterogeneous and may vary with individual-level covariates. The joint dynamics are modeled as a continuous-time Markov chain such that disease transmission is constrained by the contact network structure, and network evolution is in turn influenced by individual disease statuses. To accommodate partial epidemic observations commonly seen in real-world data, we propose a likelihood-based inference method based on the stochastic EM algorithm, introducing key innovations that include efficient conditional samplers for imputing missing infection and recovery times which respect the dynamic contact network. Experiments on both synthetic and real datasets demonstrate that our inference method can accurately and efficiently recover model parameters and provide valuable insight at the presence of unobserved disease episodes in epidemic data.

==> new_version.tex <==


The model specification in the previous section based on a CTMC with individual-level Poisson processes lends itself to the specification of a complete data likelihood for the collection of parameters in the model $\Theta = \{\beta, \varphi, \gamma, \eta, b_S, \boldsymbol\alpha, \boldsymbol\omega\}$ (where $\boldsymbol\alpha = \{\alpha_{ABk}\}_{k\in\{0,1\}, (A,B)\in \mathcal{S}}$, $ \boldsymbol\omega = \{\omega_{ABk}\}_{k\in\{0,1\}, (A,B)\in \mathcal{S}}$, and here $\mathcal{S}=\{(H,H), (H,I), (I,I)\}$ is the set of all pair types).

$$L(\Theta; \text{complete data}) = L(\Theta^N; \text{complete data})L(\Theta^E;\text{complete data})$$

\begin{align}
    & L(\Theta; \text{complete data})  \label{eq: complete-data-likelihood}\\
   &= \beta^{n_E} \gamma^{n_R} \varphi^{n_I} p_s^{n_{I_s}} (1-p_s)^{n_{I_a}} \nonumber\\
   \times & \prod_{i: i \text{ got exposed}} e^{b_S^T x_i} \left[I^{a}_i(t_i^{(E)})+I^{s}_i(t_i^{(E)}) e^{\eta}\right] \nonumber \\
    \times & \exp\left(-\int_0^T \left[\beta \sum_{i=1}^N e^{b_S^T x_i} \left[I^{a}_i(t)+I^{s}_i(t) e^{\eta}\right]\mathbbm{1}(i\text{ is susceptible at } t) + \gamma (I^a(t)+I^s(t)) + \varphi E(t)\right] dt \right)  \nonumber \\
    \times & \prod_{k=0,1}\prod_{(A,B)\in \mathcal{S}} \left[\left(\alpha_{ABk}\right)^{C_{ABk}} \left(\omega_{ABk}\right)^{D_{ABk}}\right] %\prod_{i=1}^N e^{N^c_i u_i}e^{N^d_i v_i}  
    \nonumber \\
    \times & 
    % \exp\left( -\int_0^T \sum_{i,j=1:N, i<j} \left[ \alpha_{A_{it}A_{jt}k} e^{u_i+u_j} (1-\mathbbm{1}_{i-j}(t)) + \omega_{A_{it}A_{jt}k} e^{v_i+v_j} \mathbbm{1}_{i-j}(t)\right] dt \right). 
    \exp\left( -\int_0^T  \sum_{k=0,1}\sum_{(A,B)\in \mathcal{S}} \left[ \alpha_{ABk} M^d_{AB}(t) + \omega_{ABk} M^c_{AB}(t) \right] \mathbbm{1}(t \in \mathcal{T}_k)dt \right). \nonumber
\end{align}

It is important to note that while this is a likelihood for the parameters of both the network and epidemic process, given the complete data the two processes can actually be decoupled, leading to the product form of the likelihood above. 
The first three lines of Eq~XX relate to the epidemic dynamics and the last two lines refer to the network dynamics.  
The separate components are themselves simple products of all the exponential rates for 
inter-event times related to the network and epidemic processes, respectively. More so, both epidemic and network components can be decomposed into population level and individual level contributions. 
% Some of the those inter-event rates can be considered at the population level, and so keeping track of population-level summary counts is important for evaluating the likelihood. 
For example, we need to record the total number of individuals that ever entered each status (e.g., $n_E$, total number of exposed cases), the number of individuals of each status at any time point $t$ (e.g., $E(t)$, number of $E$ people at time $t$), and the total number of link changes for each link type at each time phase (e.g., $C_{HI0}$, number of link activation events for $H$-$I$ pairs in phase $\mathcal{T}_0$). Additionally, there are inter-event rates that depend on individual-level information. For instance, to calculate the exposure rate for a susceptible individual $i$, we need to know the number of $I_a$ and $I_s$ neighbors at any time $t$, denoted by $I_i^a(t)$ and $I_i^s(t)$ respectively. Further, we denote each individual $i$'s exposure time by $t_i^{(E)}$ (set to $T$ if never exposed) and manifestation time by $t_i^{(I)}$ (set to $T$ if never exposed). 



==> old_intro_text.tex <==
\section{Introduction}
The modeling of infectious disease has traditionally relied on compartmental models, where only the disease status of an individual plays a role in understanding the disease dynamics. Examples of such mechanistic compartmental models abound in the epidemiology and mathematical biology literature (e.g. susceptible-infectious-recovered (SIR) model, \cite{kermack1927contribution}), where the vast majority of them simplify disease transmission to a population level event --- as such the question that these models can help answer about disease outbreaks are not individual level (``what is my risk of infection?'') but population level (``will the outbreak end?''). This is because many of these models introduce a ``random mixing'' assumption about the infectious population, claiming that any infected individual can transmit the disease to any other susceptible individual. However, it is clear that the contact network of individuals plays an integral role in the transmission of the disease and that interventions on individual behavior can change the overall dynamics of an outbreak. The literature on epidemics diffusing through networks has been greatly bolstered during the SARS-COV-2 pandemic, with an introduction of a myriad of transmission dynamics that are able to capture both network and individual characteristics \citep{ferguson2020report, cencetti2020using,nielsen2021covid,small2020modelling,skums2020global,lee2020engines, soriano2021household}. 

NEED TO PUT IN TWO SENTENCES TO SAY THAT THERE ARE LOTS OF OPTIONS FOR INDIVIDUAL LEVEL MODELS BUT THEY ARE MAINLY GARBAGE BECAUSE THEY SIMPLY PUT RANDOMNESS OVER THE OBSERVATION PROCESS RATHER THAN THE ACTUAL EPIDEMIC.
Building on previous work (such as \cite{auranen2000transmission,Kiss2017,clementi2010flooding,ogura2016epidemic}), \cite{bu2020likelihood} introduced an individual level network-based framework for stochastic epidemic processes, where information about infections and individual-to-individual interactions are nearly-completely observed. Specifically, the proposed modeling approach introduced an exact sampler for partially-observed recovery times while conditioning on fully observed infection times. Unfortunately, much of the available data on epidemics only provides a partial view on infection and recovery times --- and frequently obscures the differences between infection and exposure times. Because it is likely that diseases such as the flu and coronaviruses have a substantial incubation period, it is important to develop tools that can accommodate such data shortcomings. 

I THINK THIS INTRO NEEDS A PICTURE OF THE TYPE OF DATA THAT WE HAVE --- SHOWING HOW IT CAN BE PARTIALLY OBSERVED, ETC. MAYBE SIMILAR TO THE DARCI ILLUSTRATION FROM THE OTHER PAPER BUT MORE PICTORIAL.

ALSO, THIS IS AOAS SO WE NEED TO EMPHASIZE THE APPLICATION. THAT IS, THERE NEEDS TO BE A PARAGRAPH OR TWO ABOUT THE DATASET. I THINK THAT AFTER THE PARAGRAPH I PUT IN ABOUT DATA SHORTCOMINGS WE SHOULD SAY ``BTW, WE CAN ANALYZE THE DATA WITHOUT ALL OF THE FANCY STUFF WE DEVELOP IN THIS PAPER.'' WE SHOULD INCLUDE A CROSS-TAB OF INFECTED VS THE DIFFERENT COVARIATES WE MEASURE ABOUT THEM AND SAY ``LOOK, IT SEEMS THAT INFECTIONS ARE LESS LIKELY FOR PEOPLE WHO WASH THEIR HANDS --- IS THAT REAL OR IS THAT JUST GARBAGE''.



June 28: the story is as follows: we know that handwashing is important \citep{aiello2010mask,hubner2013impact,hovi2017intensified,thompson2015healthy,stedman2015outcomes,arbogast2016impact,stedman2015hand,savolainen2012hand} because we have randomized experiments for things like this. Our data are not a randomized experiment of whether handwashing is important and so it is not obvious how to assess the hypothesis that handwashing is important from our data. Raw counts/fractions suggest that handwashingt helps (people who wash their hands often get infected X percent less than those who do not) but a proportions or exact test do not really make sense since there are so many dependencies in the data (put in network picture of infections happening). Because of this it is necessary to build in the handwashing status of individuals directly into the transmission model in order to attempt to assess whether handwashing has an effect on tranmissions rates/probabilities. 


\begin{figure}[ht]
    \centering
    \includegraphics[trim=0 1in 0 0.7in, clip, width=0.9\textwidth]{figures/select_network_transmission.pdf}
    \caption{Weekly aggregated contact networks for select participants in the iEpi study. Healthy and sick individuals are marked in {\color{skyblue} \bf blue} and {\color{indianred} \bf red} respectively. Individuals who wash their hands optimally are marked by squares, while those who don't are marked by circles. Here we present the contact networks centered at person 19 from week 4 to week 7 of the study. In week 4, person 19 is infectious, and by week 5 four of his neighbors are infected; later on person 23 and person 7 keep infecting their neighbors and thus spread the disease onto person 99 and 14 by week 7. It is notable that all subsequent infections after 19 are for those who do \textbf{not} wash their hands optimally. Moreover, it appears that an individual tends to lose previous contacts after getting sick. }
    \label{fig:subnet-transmission}
\end{figure}


%\underline{Outline}: (1) infectious diseases bad, take place via interpersonal contact; (2) modern data with high-frequency observations, important questions include effects of mitigation strategy (coefficients that modulate infection rates via individual-level covariates, e.g., hand-washing), but traditional models (GLMs on the counts, etc.) are as not good as stochastic process models because...; 


\underline{Paper length limit}: 20 pages (about 500 words per page, with figures typically taking 1/3 page and displayed equations 30 words each)


